MetaCloak: Preventing Unauthorized Subject-driven Text-to-image Diffusion-based Synthesis via Meta-learning

Text-to-image diffusion models allow seamless generation of personalized images from scant reference photos. Yet, these tools, in the wrong hands, can fabricate misleading or harmful content, endangering individuals. To address this problem, existing poisoning-based approaches perturb user images in an imperceptible way to render them "unlearnable" from malicious uses. We identify two limitations of these defending approaches: i) sub-optimal due to the hand-crafted heuristics for solving the intractable bilevel optimization and ii) lack of robustness against simple data transformations like Gaussian filtering. To solve these challenges, we propose MetaCloak, which solves the bi-level poisoning problem with a meta-learning framework with an additional transformation sampling process to craft transferable and robust perturbation. Specifically, we employ a pool of surrogate diffusion models to craft transferable and model-agnostic perturbation. Furthermore, by incorporating an additional transformation process, we design a simple denoising-error maximization loss that is sufficient for causing transformation-robust semantic distortion and degradation in a personalized generation. Extensive experiments on the VGGFace2 and CelebA-HQ datasets show that MetaCloak outperforms existing approaches. Notably, MetaCloak can successfully fool online training services like Replicate, in a black-box manner, demonstrating the effectiveness of MetaCloak in real-world scenarios. Our code is available at https://github.com/liuyixin-louis/MetaCloak.

==> figs/main-compare-vis.tex <==

\begin{figure*}
    % \setlength{\tabcolsep}{1pt} % Default value: 6pt
    \setlength{\tabcolsep}{0pt} % Set this to 0pt to remove the gap
    \renewcommand{\arraystretch}{0} % Default value: 1
    \begin{center}
    \begin{tabular*}{\linewidth}
    % {cccccc}
{ccccccccc}
% \toprule
Input &ASPL & E-ASPL & T-ASPL & FSMG  & AdvDM & MetaCloak \\ 
% \midrule
 \includegraphics[width=0.14\linewidth]{figs/transformations-test/VGGFace2/48/clean_input/0.png} &
    \includegraphics[width=0.14\linewidth]{figs/transformations-test/VGGFace2/48/no-trans/ASPL/a_dslr_photo_of_rjq_person/0_0.png} &
    \includegraphics[width=0.14\linewidth]{figs/transformations-test/VGGFace2/48/no-trans/EASPL/a_dslr_photo_of_rjq_person/0_0.png} &
    \includegraphics[width=0.14\linewidth]{figs/transformations-test/VGGFace2/48/no-trans/TASPL/a_dslr_photo_of_rjq_person/0_0.png} &
    \includegraphics[width=0.14\linewidth]{figs/transformations-test/VGGFace2/48/no-trans/FSMG/a_dslr_photo_of_rjq_person/0_0.png} &
    \includegraphics[width=0.14\linewidth]{figs/transformations-test/VGGFace2/48/no-trans/AdvDM/a_dslr_photo_of_rjq_person/0_0.png} &
    \includegraphics[width=0.14\linewidth]{figs/transformations-test/VGGFace2/48/no-trans/MetaCloak/a_dslr_photo_of_rjq_person/1.png}
    \\ 

    \includegraphics[width=0.14\linewidth]{figs/transformations-test/VGGFace2/48/clean_input/1.png} & \includegraphics[width=0.14\linewidth]{
    figs/transformations-test/VGGFace2/48/gua/7/ASPL/a_dslr_photo_of_rjq_person/0.png
 } &
 \includegraphics[width=0.14\linewidth]{
    figs/transformations-test/VGGFace2/48/gua/7/EASPL/a_dslr_photo_of_rjq_person/0.png
 } &
 \includegraphics[width=0.14\linewidth]{
    figs/transformations-test/VGGFace2/48/gua/7/TASPL/a_dslr_photo_of_rjq_person/0.png 
 } &
 \includegraphics[width=0.14\linewidth]{
    figs/transformations-test/VGGFace2/48/gua/7/FSMG/a_dslr_photo_of_rjq_person/0.png
 } &
 \includegraphics[width=0.14\linewidth]{
    figs/transformations-test/VGGFace2/48/gua/7/AdvDM/a_dslr_photo_of_rjq_person/0.png
 } &
 \includegraphics[width=0.14\linewidth]{
    figs/transformations-test/VGGFace2/48/gua/7/MetaCloak/a_dslr_photo_of_rjq_person/0.png
 } \\

    \end{tabular*}
    \caption{
        Transformation robustness of different methods. The first row is a generated sample from DreamBooth trained on poisons with no transformation defenses. The 2-th row showcases the robustness of each method under transformation with a Gaussian kernel size of 7. Our method performs robustly under transformation defenses, while other methods fail to preserve the perturbation.
    }
    \label{fig:main.compare.vis}
    \end{center}
\end{figure*}


==> pre.tex <==
%
%
% Commonly used packages, definitions, and notations
%
% Yixin Liu
% yixinliucs@gmail.com
%
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% commonly used packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\let\proof\relax
\let\endproof\relax
\let\amalg\relax

\newcommand\hmmax{0}
\newcommand\bmmax{0}
\usepackage{xspace}

\usepackage{amsthm}
\theoremstyle{definition}


\usepackage{epsfig,amsmath,amsfonts,epsfig,multirow,makecell,caption,soul,csquotes,subcaption,mathtools,bm,spverbatim,booktabs,tcolorbox,diagbox,todonotes}
\usepackage[e]{esvect}


\newcommand{\btodo}[1]{\todo[fancyline, inline, bordercolor=white, color=yellow!40]{#1}}
\newcommand{\rtodo}[1]{{\color{red}{#1}}}

\usepackage{latexsym}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{mathrsfs}
\usepackage{url}


%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\newcommand{\mfe}{\mathfrak{e}}
\newcommand{\mfb}{\mathfrak{b}}


\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\phib}{\boldsymbol{\phi}}
\newcommand{\omegab}{\boldsymbol{\omega}}

\newcommand{\Phib}{\boldsymbol{\Phi}}
% \newcommand{\ab}{\bm{a}}
% \newcommand{\bb}{\bm{b}}
% \newcommand{\cbb}{\bm{c}}
% \newcommand{\db}{\bm{d}}
% \newcommand{\eb}{\bm{e}}
% \newcommand{\fb}{\bm{f}}
% \newcommand{\gb}{\bm{g}}
% \newcommand{\hb}{\bm{h}}
% \newcommand{\ib}{\bm{i}}
% \newcommand{\jb}{\bm{j}}
% \newcommand{\kb}{\bm{k}}
% \newcommand{\lb}{\bm{l}}
% \newcommand{\mb}{\bm{m}}
% \newcommand{\nbb}{\bm{n}}
% \newcommand{\ob}{\bm{o}}
% \newcommand{\pb}{\bm{p}}
% \newcommand{\qb}{\bm{q}}
% \newcommand{\rb}{\bm{r}}
% \newcommand{\sbb}{\bm{s}}
% \newcommand{\tb}{\bm{t}}
% \newcommand{\ub}{\bm{u}}
% \newcommand{\vb}{\bm{v}}
% \newcommand{\wb}{\bm{w}}
% \newcommand{\xb}{\bm{x}}
% \newcommand{\yb}{\bm{y}}
% \newcommand{\zb}{\bm{z}}

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\abtil}{\tilde{\ab}}
\newcommand{\bbtil}{\tilde{\bb}}
\newcommand{\cbtil}{\tilde{\cbb}}
\newcommand{\dbtil}{\tilde{\db}}
\newcommand{\ebtil}{\tilde{\eb}}
\newcommand{\fbtil}{\tilde{\fb}}
\newcommand{\gbtil}{\tilde{\gb}}
\newcommand{\hbtil}{\tilde{\hb}}
\newcommand{\ibtil}{\tilde{\ib}}
\newcommand{\jbtil}{\tilde{\jb}}
\newcommand{\kbtil}{\tilde{\kb}}
\newcommand{\lbtil}{\tilde{\lb}}
\newcommand{\mbtil}{\tilde{\mb}}
\newcommand{\nbtil}{\tilde{\nbb}}
\newcommand{\obtil}{\tilde{\ob}}
\newcommand{\pbtil}{\tilde{\pb}}
\newcommand{\qbtil}{\tilde{\qb}}
\newcommand{\rbtil}{\tilde{\rb}}
\newcommand{\sbtil}{\tilde{\sbb}}
\newcommand{\tbtil}{\tilde{\tb}}
\newcommand{\ubtil}{\tilde{\ub}}
\newcommand{\vbtil}{\tilde{\vb}}
\newcommand{\wbtil}{\tilde{\wb}}
\newcommand{\xbtil}{\tilde{\xb}}
\newcommand{\ybtil}{\tilde{\yb}}
\newcommand{\zbtil}{\tilde{\zb}}


\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\obar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\abbar}{\bar{\ab}}
\newcommand{\bbbar}{\bar{\bb}}
\newcommand{\cbbar}{\bar{\cb}}
\newcommand{\dbbar}{\bar{\db}}
\newcommand{\ebbar}{\bar{\eb}}
\newcommand{\fbbar}{\bar{\fb}}
\newcommand{\gbbar}{\bar{\gb}}
\newcommand{\hbbar}{\bar{\hb}}
\newcommand{\ibbar}{\bar{\ib}}
\newcommand{\jbbar}{\bar{\jb}}
\newcommand{\kbbar}{\bar{\kb}}
\newcommand{\lbbar}{\bar{\lb}}
\newcommand{\mbbar}{\bar{\mb}}
\newcommand{\nbbar}{\bar{\nbb}}
\newcommand{\obbar}{\bar{\ob}}
\newcommand{\pbbar}{\bar{\pb}}
\newcommand{\qbbar}{\bar{\qb}}
\newcommand{\rbbar}{\bar{\rb}}
\newcommand{\sbbar}{\bar{\sbb}}
\newcommand{\tbbar}{\bar{\tb}}
\newcommand{\ubbar}{\bar{\ub}}
\newcommand{\vbbar}{\bar{\vb}}
\newcommand{\wbbar}{\bar{\wb}}
\newcommand{\xbbar}{\bar{\xb}}
\newcommand{\ybbar}{\bar{\yb}}
\newcommand{\zbbar}{\bar{\zb}}

% \newcommand{\Ab}{\bm{A}}
% \newcommand{\Bb}{\bm{B}}
% \newcommand{\Cb}{\bm{C}}
% \newcommand{\Db}{\bm{D}}
% \newcommand{\Eb}{\bm{E}}
% \newcommand{\Fb}{\bm{F}}
% \newcommand{\Gb}{\bm{G}}
% \newcommand{\Hb}{\bm{H}}
% \newcommand{\Ib}{\bm{I}}
% \newcommand{\Jb}{\bm{J}}
% \newcommand{\Kb}{\bm{K}}
% \newcommand{\Lb}{\bm{L}}
% \newcommand{\Mb}{\bm{M}}
% \newcommand{\Nb}{\bm{N}}
% \newcommand{\Ob}{\bm{O}}
% \newcommand{\Pb}{\bm{P}}
% \newcommand{\Qb}{\bm{Q}}
% \newcommand{\Rb}{\bm{R}}
% \newcommand{\Sbb}{\bm{S}}
% \newcommand{\Tb}{\bm{T}}
% \newcommand{\Ub}{\bm{U}}
% \newcommand{\Vb}{\bm{V}}
% \newcommand{\Wb}{\bm{W}}
% \newcommand{\Xb}{\bm{X}}
% \newcommand{\Yb}{\bm{Y}}
% \newcommand{\Zb}{\bm{Z}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

% \newcommand{\Abtil}{\tilde{\Ab}}
% \newcommand{\Bbtil}{\tilde{\Bb}}
% \newcommand{\Cbtil}{\tilde{\Cb}}
% \newcommand{\Dbtil}{\tilde{\Db}}
% \newcommand{\Ebtil}{\tilde{\Eb}}
% \newcommand{\Fbtil}{\tilde{\Fb}}
% \newcommand{\Gbtil}{\tilde{\Gb}}
% \newcommand{\Hbtil}{\tilde{\Hb}}
% \newcommand{\Ibtil}{\tilde{\Ib}}
% \newcommand{\Jbtil}{\tilde{\Jb}}
% \newcommand{\Kbtil}{\tilde{\Kb}}
% \newcommand{\Lbtil}{\tilde{\Lb}}
% \newcommand{\Mbtil}{\tilde{\Mb}}
% \newcommand{\Nbtil}{\tilde{\Nb}}
% \newcommand{\Obtil}{\tilde{\Ob}}
% \newcommand{\Pbtil}{\tilde{\Pb}}
% \newcommand{\Qbtil}{\tilde{\Qb}}
% \newcommand{\Rbtil}{\tilde{\Rb}}
% \newcommand{\Sbtil}{\tilde{\Sbb}}
% \newcommand{\Tbtil}{\tilde{\Tb}}
% \newcommand{\Ubtil}{\tilde{\Ub}}
% \newcommand{\Vbtil}{\tilde{\Vb}}
% \newcommand{\Wbtil}{\tilde{\Wb}}
% \newcommand{\Xbtil}{\tilde{\Xb}}
% \newcommand{\Ybtil}{\tilde{\Yb}}
% \newcommand{\Zbtil}{\tilde{\Zb}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\Ahat}{\widehat{A}}
\newcommand{\Bhat}{\widehat{B}}
\newcommand{\Chat}{\widehat{C}}
\newcommand{\Dhat}{\widehat{D}}
\newcommand{\Ehat}{\widehat{E}}
\newcommand{\Fhat}{\widehat{F}}
\newcommand{\Ghat}{\widehat{G}}
\newcommand{\Hhat}{\widehat{H}}
\newcommand{\Ihat}{\widehat{I}}
\newcommand{\Jhat}{\widehat{J}}
\newcommand{\Khat}{\widehat{K}}
\newcommand{\Lhat}{\widehat{L}}
\newcommand{\Mhat}{\widehat{M}}
\newcommand{\Nhat}{\widehat{N}}
\newcommand{\Ohat}{\widehat{O}}
\newcommand{\Phat}{\widehat{P}}
\newcommand{\Qhat}{\widehat{Q}}
\newcommand{\Rhat}{\widehat{R}}
\newcommand{\Shat}{\widehat{S}}
\newcommand{\That}{\widehat{T}}
\newcommand{\Uhat}{\widehat{U}}
\newcommand{\Vhat}{\widehat{V}}
\newcommand{\What}{\widehat{W}}
\newcommand{\Xhat}{\widehat{X}}
\newcommand{\Yhat}{\widehat{Y}}
\newcommand{\Zhat}{\widehat{Z}}

\newcommand{\ahat}{\widehat{a}}
\newcommand{\bhat}{\widehat{b}}
\newcommand{\chat}{\widehat{c}}
\newcommand{\dhat}{\widehat{d}}
\newcommand{\ehat}{\widehat{e}}
\newcommand{\fhat}{\widehat{f}}
\newcommand{\ghat}{\widehat{g}}
\newcommand{\hhat}{\widehat{h}}
\newcommand{\ihat}{\widehat{i}}
\newcommand{\jhat}{\widehat{j}}
\newcommand{\khat}{\widehat{k}}
\newcommand{\lhat}{\widehat{l}}
\newcommand{\mhat}{\widehat{m}}
\newcommand{\nhat}{\widehat{n}}
\newcommand{\ohat}{\widehat{o}}
\newcommand{\phat}{\widehat{p}}
\newcommand{\qhat}{\widehat{q}}
\newcommand{\rhat}{\widehat{r}}
\newcommand{\shat}{\widehat{s}}
\newcommand{\that}{\widehat{t}}
\newcommand{\uhat}{\widehat{u}}
\newcommand{\vhat}{\widehat{v}}
\newcommand{\what}{\widehat{w}}
\newcommand{\xhat}{\widehat{x}}
\newcommand{\yhat}{\widehat{y}}
\newcommand{\zhat}{\widehat{z}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\Ascr}{\mathscr{A}}
\newcommand{\Bscr}{\mathscr{B}}
\newcommand{\Cscr}{\mathscr{C}}
\newcommand{\Dscr}{\mathscr{D}}
\newcommand{\Escr}{\mathscr{E}}
\newcommand{\Fscr}{\mathscr{F}}
\newcommand{\Gscr}{\mathscr{G}}
\newcommand{\Hscr}{\mathscr{H}}
\newcommand{\Iscr}{\mathscr{I}}
\newcommand{\Jscr}{\mathscr{J}}
\newcommand{\Kscr}{\mathscr{K}}
\newcommand{\Lscr}{\mathscr{L}}
\newcommand{\Mscr}{\mathscr{M}}
\newcommand{\Nscr}{\mathscr{N}}
\newcommand{\Oscr}{\mathscr{O}}
\newcommand{\Pscr}{\mathscr{P}}
\newcommand{\Qscr}{\mathscr{Q}}
\newcommand{\Rscr}{\mathscr{R}}
\newcommand{\Sscr}{{\mathscr{S}}}
\newcommand{\Tscr}{{\mathscr{T}}}
\newcommand{\Uscr}{\mathscr{U}}
\newcommand{\Vscr}{\mathscr{V}}
\newcommand{\Wscr}{\mathscr{W}}
\newcommand{\Xscr}{\mathscr{X}}
\newcommand{\Yscr}{\mathscr{Y}}
\newcommand{\Zscr}{\mathscr{Z}}

\newcommand{\Afra}{\mathfrak{A}}
\newcommand{\Bfra}{\mathfrak{B}}
\newcommand{\Cfra}{\mathfrak{C}}
\newcommand{\Dfra}{\mathfrak{D}}
\newcommand{\Efra}{\mathfrak{E}}
\newcommand{\Ffra}{\mathfrak{F}}
\newcommand{\Gfra}{\mathfrak{G}}
\newcommand{\Hfra}{\mathfrak{H}}
\newcommand{\Ifra}{\mathfrak{I}}
\newcommand{\Jfra}{\mathfrak{J}}
\newcommand{\Kfra}{\mathfrak{K}}
\newcommand{\Lfra}{\mathfrak{L}}
\newcommand{\Mfra}{\mathfrak{M}}
\newcommand{\Nfra}{\mathfrak{N}}
\newcommand{\Ofra}{\mathfrak{O}}
\newcommand{\Pfra}{\mathfrak{P}}
\newcommand{\Qfra}{\mathfrak{Q}}
\newcommand{\Rfra}{\mathfrak{R}}
\newcommand{\Sfra}{{\mathfrak{S}}}
\newcommand{\Tfra}{{\mathfrak{T}}}
\newcommand{\Ufra}{\mathfrak{U}}
\newcommand{\Vfra}{\mathfrak{V}}
\newcommand{\Wfra}{\mathfrak{W}}
\newcommand{\Xfra}{\mathfrak{X}}
\newcommand{\Yfra}{\mathfrak{Y}}
\newcommand{\Zfra}{\mathfrak{Z}}


\newcommand{\Acalb}{\bm{\Acal}}
\newcommand{\Bcalb}{\bm{\Bcal}}
\newcommand{\Ccalb}{\bm{\Ccal}}
\newcommand{\Dcalb}{\bm{\Dcal}}
\newcommand{\Ecalb}{\bm{\Ecal}}
\newcommand{\Fcalb}{\bm{\Fcal}}
\newcommand{\Gcalb}{\bm{\Gcal}}
\newcommand{\Hcalb}{\bm{\Hcal}}
\newcommand{\Icalb}{\bm{\Ical}}
\newcommand{\Jcalb}{\bm{\Jcal}}
\newcommand{\Kcalb}{\bm{\Kcal}}
\newcommand{\Lcalb}{\bm{\Lcal}}
\newcommand{\Mcalb}{\bm{\Mcal}}
\newcommand{\Ncalb}{\bm{\Ncal}}
\newcommand{\Ocalb}{\bm{\Ocal}}
\newcommand{\Pcalb}{\bm{\Pcal}}
\newcommand{\Qcalb}{\bm{\Qcal}}
\newcommand{\Rcalb}{\bm{\Rcal}}
\newcommand{\Scalb}{\bm{\Scal}}
\newcommand{\Tcalb}{\bm{\Tcal}}
\newcommand{\Ucalb}{\bm{\Ucal}}
\newcommand{\Vcalb}{\bm{\Vcal}}
\newcommand{\Wcalb}{\bm{\Wcal}}
\newcommand{\Xcalb}{\bm{\Xcal}}
\newcommand{\Ycalb}{\bm{\Ycal}}
\newcommand{\Zcalb}{\bm{\Zcal}}

\newcommand{\Ascrb}{\bm{\Ascr}}
\newcommand{\Bscrb}{\bm{\Bscr}}
\newcommand{\Cscrb}{\bm{\Cscr}}
\newcommand{\Dscrb}{\bm{\Dscr}}
\newcommand{\Escrb}{\bm{\Escr}}
\newcommand{\Fscrb}{\bm{\Fscr}}
\newcommand{\Gscrb}{\bm{\Gscr}}
\newcommand{\Hscrb}{\bm{\Hscr}}
\newcommand{\Iscrb}{\bm{\Iscr}}
\newcommand{\Jscrb}{\bm{\Jscr}}
\newcommand{\Kscrb}{\bm{\Kscr}}
\newcommand{\Lscrb}{\bm{\Lscr}}
\newcommand{\Mscrb}{\bm{\Mscr}}
\newcommand{\Nscrb}{\bm{\Nscr}}
\newcommand{\Oscrb}{\bm{\Oscr}}
\newcommand{\Pscrb}{\bm{\Pscr}}
\newcommand{\Qscrb}{\bm{\Qscr}}
\newcommand{\Rscrb}{\bm{\Rscr}}
\newcommand{\Sscrb}{\bm{\Sscr}}
\newcommand{\Tscrb}{\bm{\Tscr}}
\newcommand{\Uscrb}{\bm{\Uscr}}
\newcommand{\Vscrb}{\bm{\Vscr}}
\newcommand{\Wscrb}{\bm{\Wscr}}
\newcommand{\Xscrb}{\bm{\Xscr}}
\newcommand{\Yscrb}{\bm{\Yscr}}
\newcommand{\Zscrb}{\bm{\Zscr}}

\newcommand{\Afrab}{\bm{\Afra}}
\newcommand{\Bfrab}{\bm{\Bfra}}
\newcommand{\Cfrab}{\bm{\Cfra}}
\newcommand{\Dfrab}{\bm{\Dfra}}
\newcommand{\Efrab}{\bm{\Efra}}
\newcommand{\Ffrab}{\bm{\Ffra}}
\newcommand{\Gfrab}{\bm{\Gfra}}
\newcommand{\Hfrab}{\bm{\Hfra}}
\newcommand{\Ifrab}{\bm{\Ifra}}
\newcommand{\Jfrab}{\bm{\Jfra}}
\newcommand{\Kfrab}{\bm{\Kfra}}
\newcommand{\Lfrab}{\bm{\Lfra}}
\newcommand{\Mfrab}{\bm{\Mfra}}
\newcommand{\Nfrab}{\bm{\Nfra}}
\newcommand{\Ofrab}{\bm{\Ofra}}
\newcommand{\Pfrab}{\bm{\Pfra}}
\newcommand{\Qfrab}{\bm{\Qfra}}
\newcommand{\Rfrab}{\bm{\Rfra}}
\newcommand{\Sfrab}{\bm{\Sfra}}
\newcommand{\Tfrab}{\bm{\Tfra}}
\newcommand{\Ufrab}{\bm{\Ufra}}
\newcommand{\Vfrab}{\bm{\Vfra}}
\newcommand{\Wfrab}{\bm{\Wfra}}
\newcommand{\Xfrab}{\bm{\Xfra}}
\newcommand{\Yfrab}{\bm{\Yfra}}
\newcommand{\Zfrab}{\bm{\Zfra}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}


%%%%%%%% Widely accepted definitions %%%%%%%%%%%%%%%

\newcommand{\BB}{\mathbb{B}} % Complex numbers
\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\II}{\mathbb{I}} % Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\LL}{\mathbb{L}} % Loss
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\ZZ}{\mathbb{Z}} % Integers
\newcommand{\XX}{\mathbb{X}} %
\newcommand{\YY}{\mathbb{Y}} %

\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
%\newcommand{\TRUE}{\mathbf{TRUE}}  % True
%\newcommand{\FALSE}{\mathbf{FALSE}}  % False

\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
% \newcommand*{\st}{\mathop{\mathrm{s.t.}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\ovec}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand*{\cov}{\mathrm{Cov}}
\newcommand*{\conv}{\mathrm{conv}}
\newcommand*{\const}{\mathrm{constant}}

%%%%%%%% Bold Greek Letters %%%%%%%%%%%%%%%
\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}


%%%%%%%% Mess around with LaTeX %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
%\newenvironment{proof}{\emph{Proof. }}{ \hfill \QED}
\fi

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
% \newtheorem{property}{Property}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\fi

\ifx\axiom\undefined
\newtheorem{axiom}[theorem]{Axiom}
\fi

%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\sembrack}[1]{[\![#1]\!]}

\def\etal{\emph{et al.}}
% \newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\emph{i.i.d.}}
\newcommand{\etc}{\emph{etc.}}

%\newcommand{\alex}[1]{{\bf ALEX: \uppercase{#1}}}
%\newcommand{\vishy}[1]{{\bf VISHY: \uppercase{#1}}}
%\newcommand{\rene}[1]{{\bf RENE: \uppercase{#1}}}
%\newcommand{\karsten}[1]{{\bf KARSTEN: \uppercase{#1}}}

%%%%%%%% Specific symbols for this project %%%%%%%%%%%%%%%

\newcommand{\methodname}{KDE}
\newcommand{\ind}{\boldsymbol{\mathsf{I}}}

\newcommand{\hsic}{\mathrm{HSIC}}
\newcommand{\mmd}{\mathrm{MMD}}

%\newcommand{\tDiag}{\textsf{Diag}}
%\newcommand{\tTr}{\textsf{Tr}}
%\newcommand{\tE}{\textsf{E}}
%\newcommand{\tVec}{\textsf{Vec}}
%\newcommand{\tRank}{\textsf{Rank}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% math symbols and commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\eq}[1]{(\ref{#1})}
%\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}

%brackets
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\renewcommand{\url}[1]{{\sffamily #1}}
\newcommand{\arow}[2]{#1_{#2\cdot}}
\newcommand{\acol}[2]{#1_{\cdot#2}}
\def\ci{\perp\!\!\!\perp}

\newcommand{\ssbr}[1]{\left[\!\left[#1\right]\!\right]}

\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}

\newcommand{\wtimes}[1]{\times_{#1}}
\newcommand{\btimes}[1]{~\bar{\times}_{#1}~}


%%%%%%%%%% commonly-used notations
\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}
\def \ee {{\bm{e}}}
\def \rr {{\bm{r}}}
\def \xx {{\bm{x}}}
\def \yy {{\bm{y}}}
\def \pp {{\bm{p}}}
\def \qq {{\bm{q}}}
\def \uu {{\bm{u}}}
\def \ww {{\bm{w}}}
\def \zz {{\bm{z}}}
\def \ej {{\bm{e_j}}}
\def \ei {{\bm{e_i}}}
\def \btheta {{\bm{\theta}}}
% \def \X  {\mathcal{X}}
% \def \Y  {\mathcal{Y}}
% \def \F  {\mathcal{F}}
% \def \H  {\mathcal{H}}
% \def \L  {\mathcal{L}}
% \def \R  {\mathbb{R}}
% \def \U  {\mathcal{U}}
% \def \D  {\mathcal{D}}
% \def \C  {\mathcal{C}}
% \def \F  {\mathcal{F}}
% \def \E  {\mathbb{E}}
\def \gnn {{GNN}}
\def \gnns {{GNNs}}
\newcommand{\header}[1]{\noindent\textbf{#1}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% space trick
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\ssup}[2]{{#1}^{{#2}}}
\newcommand{\ssub}[2]{{#1}_{{#2}}}
\newcommand{\sboth}[3]{{#1}_{{#2}}^{{#3}}}


==> sections/reproduciblity_checklist.tex <==
\section{Reproducibility Checklist}

This paper

\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced. \textbf{Yes. See page 4 of the main text.}
    \item Clearly delineates statements that are opinions, hypotheses, and speculation from objective facts and results. \textbf{Yes.}
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper. \textbf{Yes.}
    \item Does this paper make theoretical contributions? \textbf{No.}
    \item If yes, please complete the list below. \textbf{Theory checklist Not Applicable, so omitted.}


\item Does this paper rely on one or more datasets? \textbf{Yes.}
\item If yes, please complete the list below.
\begin{itemize}
    \item     A motivation is given for why the experiments are conducted on the selected datasets. \textbf{Yes. Datasets like RealToxicityPrompts and the red-teaming prompts from \citet{ganguli2022red} are standard datasets for testing harmful outputs. The human evaluation data was conducted through standard red-teaming practices where the labelers were instructed to prompt the model to produce harmful behavior. The training set of adversarial examples was generated by probing the early LLaMA-1 (Touvron et al. 2023a) model, which does not has safety alignment in place. The content of this corpus can be
found in our supplementary materials. }
    \item All novel datasets introduced in this paper are included in a data appendix. \textbf{Yes.}
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textbf{Yes.}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \textbf{Yes}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \textbf{Yes.}
    \item All datasets that are not publicly available are described in detail, with an explanation of why publicly available alternatives are not scientifically satisficing. \textbf{NA.}
\end{itemize}
\item Does this paper include computational experiments? \textbf{Yes.}
\item If yes, please complete the list below.

\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. \textbf{Yes.}
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. \textbf{Yes.}
    \item     All source codes required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textbf{Yes.}
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. \textbf{Yes.}
    \item     If an algorithm depends on randomness, then the method used for setting seeds is described sufficiently to allow results replication. \textbf{Yes.}
    \item     This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \textbf{Yes. See Appendix C.}
    \item This paper formally describes the evaluation metrics used and explains the motivation for choosing these metrics. \textbf{Yes.}
    \item This paper states the number of algorithm runs used to compute each reported result. \textbf{Yes. We report standard deviation when intervals are reported and the main text has the number of trials.} 
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \textbf{Yes.}
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \textbf{Yes. We provide treatment effects with standard deviations as opposed to focusing on significance testing.}
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. \textbf{Yes. See Appendix C.} 
    \item  This paper states the number and range of values tried per (hyper-) parameter during the development of the paper, along with the criterion used for selecting the final parameter setting. \textbf{Yes. Appendix C states the reasoning for hyperparameters. All variations tested are reported in ablations across the Appendix.}
\end{itemize}
    




\end{itemize}







==> tab/across_models.tex <==


\begin{table}[h]
    \centering
    \resizebox{0.7\linewidth}{!}{
\begin{tabular}{ccccccc} 
\toprule
Settings                                                                    & Models   & SDS $\downarrow$                       & $IMS_{\text{CLIP}}$    $\downarrow$      & $IMS_{\text{VGGNet}}$  $\downarrow$     & CLIP-IQAC $\downarrow$                   & LIQE $\downarrow$       \\
\midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Stand.\\Training\end{tabular}} & 
SD21base & \textbf{0.296}  & 0.662 & -0.051  & -0.380 & \textbf{0.180}  \\
                                                                            & SD21     &  0.220   & 0.688   & -0.186  & -0.404 & 0.172  \\
                                                                            & SDv1-5   & \\
\midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Trans. \\Training\end{tabular}} 
 & SD21base & \textbf{0.432}  & \textbf{0.644}  & \textbf{-0.151}  & \textbf{-0.440} & \textbf{0.570} \\
                                                                            & SD21      & 0.858  & 0.774  & -0.011  & 0.109  & 0.508 \\

                                                                            & SDv1-5   & 0.817            & 0.721                & 0.231                 & 0.532                & 0.708                \\
\bottomrule
\end{tabular}
    }
    \caption{
     Effectiveness of MetaCloak across different diffusion architectures. Stable Diffusion v1-5, v2-1-base, and v2-1 are abbreviated as SDv1-5, SD21base, and SD21 respectively. 
    } 
    \label{tab:diff.arch.main.table}
\end{table}

